Metasurface-controlled high-speed tunable external cavity lasers

Tunable lasers are essential for optical communication, spectroscopy, and precision sensing, where flexible and fast control of the laser wavelength is needed. However, conventional tunable laser systems often rely on mechanical actuation, which limits their tuning speed, stability, and repeatability. Alternative tuning methods, such as adjusting the temperature of the gain medium or the injection current, are either slow or suffer from unwanted coupling between frequency and intensity. Electro-optic modulators implemented after the laser offer fast frequency tunability but these components are bulky and prone to high insertion losses. Here, we introduce an external cavity semiconductor laser that achieves ultrafast frequency and amplitude tunability within a compact footprint without any moving parts. The laser employs a resonant electro-optic metasurface as the external mirror, providing narrowband feedback that enables simultaneous single-mode operation and voltage-controlled tuning across a wide range of currents. Leveraging a narrow linewidth design, we demonstrate mode-hop-free linear frequency tuning with rates of up to 70 THz/s, and frequency excursions reaching 110 MHz under a 10 V peak RF drive, clearly surpassing rates attainable through mechanical actuation. Moreover, by biasing the laser near its threshold, our platform enables intensity modulation with an efficiency above 100% at a peak voltage of 4 V. These results highlight the platform's potential for applications requiring high-speed and mode-hop-free tunable lasers, such as free-space optical communication, laser ranging, and high-resolution spectroscopy.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
